Symbolic Abstractions for Quantum Protocol Verification

Quantum protocols such as the BB84 Quantum Key Distribution protocol exchange qubits to achieve information-theoretic security guarantees. Many variants thereof were proposed, some of them being already deployed. Existing security proofs in that field are mostly tedious, error-prone pen-and-paper proofs of the core protocol only that rarely account for other crucial components such as authentication. This calls for formal and automated verification techniques that exhaustively explore all possible intruder behaviors and that scale well. The symbolic approach offers rigorous, mathematical frameworks and automated tools to analyze security protocols. Based on well-designed abstractions, it has allowed for large-scale formal analyses of real-life protocols such as TLS 1.3 and mobile telephony protocols. Hence a natural question is: Can we use this successful line of work to analyze quantum protocols? This paper proposes a first positive answer and motivates further research on this unexplored path.

==> tam_csf.tex <==
\subsubsection{Preliminaries}
\label{sec:verif:tam:prem}
To verify 5G AKA, we used the \tamarin prover~\cite{schmidt2012automated}.
\tamarin is a state-of-the-art protocol verification tool for the \emph{symbolic model}, which supports stateful protocols, a high level of automation, and equivalence properties~\cite{tamarin-equiv}, which are necessary to model privacy properties such as unlinkability.
It has previously been applied to real-world protocols with complex state machines, numerous messages, and complex security properties such as TLS 1.3~\cite{tamarin-tls}.
Moreover, it was recently extended with support for XOR~\cite{tamarin-xor}, a key ingredient for faithfully analyzing 5G AKA.
We chose \tamarin as it is currently the only tool that combines all these features, which are essential for a detailed analysis of 5G AKA.

In the symbolic model and a fortiori in \tamarin,
messages are described as terms. For example, $\exenc(m,k)$ represents the message $m$ encrypted using the key $k$.
The algebraic properties of the cryptographic functions are then specified using equations over terms.
For example the equation $\exdec(\exenc(m,k),k) = m$ specifies the expected semantics for symmetric encryption:
the decryption using the encryption key yields the plaintext.
As is common in the symbolic model, cryptographic messages do not satisfy other properties than those intended algebraic properties,
yielding the so-called \emph{black box cryptography assumption}
%%\jannik{perfect cryptography assumption?}
(\eg one cannot exploit potential weaknesses in cryptographic primitives).

The protocol itself is described using multi-set rewrite rules.
These rules manipulate multisets of \emph{facts}, which model the current state of the system with \emph{terms} as arguments.
\begin{example}\label{ex:hashmsr}
%\lum{LH: Usefulness of the example? Drop it? RS: I think *SOME* example is required - and I do not think a full (n)inj agree is suitable. JD: I fear that this example is too complicated, it requires the distinction between linear and persistent facts, and the use of pattern matching to decrypt may be counterintuitive. I know that the previous example was very light, but avoided these issues as there was no need for a shared key.}
The following rules describe a simple protocol that sends an encrypted message.
The first rule creates a new long-term shared key $k$ (the fact $\factStyle{!Ltk}$ is persistent: it can be used as a premise
multiple times).
The second rule describes the agent $A$ who sends a fresh message $m$ together with its MAC with the shared key $k$ to $B$.
Finally, the third rule describes $B$ who is expecting a message and a corresponding MAC with $k$ as input.
Note that the third rule can only be triggered if the input matches the premise, \ie if the input message is correctly MACed with $k$.
\[
\begin{array}{l}
Create\_Ltk : ~ [\factStyle{Fr}(k)] \rwr[] [\factStyle{!Ltk}(k)], \\
Send\_A : ~ [\factStyle{!Ltk}(k), \factStyle{Fr}(m)] \rwr[\factStyle{Sent}(m)] [\factStyle{Out}(\pair{m,\mac(m,k)})], \\
Receive\_B : ~ [\factStyle{!Ltk}(k), \factStyle{In}(\pair{m,\mac(m,k)})] \rwr[\factStyle{Received}(x)] [] \qed\\
\end{array}
\]
\end{example}
\looseness=-1
These rules yield a labeled transition system describing the possible protocol executions (see~\cite{tamarin-manual,schmidt2012automated} for  the syntax and semantics).
\tamarin combines the protocol semantics with a Dolev-Yao~\cite{DY81} style attacker.
This attacker controls the entire network and can thereby intercept, delete, modify, delay, inject, and build new messages.
However, he is limited by the cryptography: he cannot forge signatures or decrypt messages without knowing the key (black box  cryptography assumption).
He nevertheless can apply any function (e.g., hashing, XOR, encryption, pairing, \ldots) on messages he knows to compute new messages.

\subsubsection{Formalizing Security Goals in Tamarin}
\label{sec:formal:prop}

In \tamarin, security properties are specified in two different ways.
First, trace properties, such as secrecy or variants of authentication, are specified using formulas in a first-order logic with timepoints.
\begin{example}\label{ex:property}
Consider the multiset rewrite rules given in Example~\ref{ex:hashmsr}.
The following property specifies a form of non-injective agreement on the message,
\ie that any message received by $B$ was previously sent by $A$:
\\[0pt]\null\hfill$
% \begin{equation*}
    %\forall i:\tempsort,m:\msgsort.
    \forall i,m.
    \mathit{Received}(m)@i
    \Rightarrow ( \exists j .  \mathit{Sent}(m)@j \wedge j \lessdot i) .
  % \end{equation*}
$\hfill\null\\[2pt]
    Since the 5G AKA protocol features multiple roles and multiple instantiations thereof, agreement properties additionally require that the views of the two partners
  (who is playing which role, and what is the identity of the partner) actually match; see \Cref{ap:taxonomy}.
%% \lum{tricky: example above is rather weak as we do not check that views on identities of partners actally match.
%%   Do we want to give an example of a full ni-agreement property here? Or drop this? Or this extra sentence is enough? RS: full niag is too much. This should be enough!}
\end{example}
For each specified property, \tamarin checks that the property holds for all possible protocol executions, and all possible adversary behaviors.
To achieve this, \tamarin explores all possible executions in a
backward manner, searching for reachable attack states, which are counterexamples to the security properties.

Equivalence properties, such as unlinkability, are expressed by requiring that two instances of the protocol cannot be distinguished by the attacker.
Such properties are specified using \emph{diff}-terms
(which take two arguments), essentially defining two different instances of the protocol that only differ in some terms.
\tamarin then checks observational equivalence (see~\cite{tamarin-equiv}), i.e., it compares the two resulting systems and checks that the attacker cannot distinguish them for any execution and for any of its behaviors.

\looseness=-1
In fully automatic mode, \tamarin  either returns a proof that the property holds, or a counterexample/attack if the property is violated, or may not terminate as the underlying problem is undecidable.
\tamarin can also be used in interactive mode, where the user can guide the proof search.
Moreover the user can supply heuristics called \emph{oracles} to guide the proof search in a sound way.
We heavily rely on heuristics in our analyses as they allow us to tame the complexity of the protocol, as explained below.

